Modeling unsteady loads on wind-turbine blade sections from periodic structural oscillations and impinging gusts

Many traditional methods for wind turbine design and analysis assume quasi-steady aerodynamics, but atmospheric flows are inherently unsteady and modern turbine blades are susceptible to aeroelastic deformations. This study therefore evaluates the effectiveness of simple analytical models for capturing the effects of such unsteady conditions on wind-turbine blades. We consider a pitching and plunging airfoil in a periodic transverse gust as an idealization of unsteady loading scenarios on a blade section. A potential-flow model derived from a linear combination of canonical problems is proposed to predict the unsteady lift on a two-dimensional airfoil in the small-perturbation limit. We then perform high-fidelity two-dimensional numerical simulations of a NACA-0012 airfoil over a range of periodic pitch, plunge, and gust disturbances, and quantify the amplitude and phase of the unsteady lift response. Good agreement with the model predictions is found for low to moderate forcing amplitudes and frequencies, while deviations are observed when the angle-of-attack amplitudes approach the static flow-separation limit of the airfoil. Potential explanations are given for the cases in which the ideal-flow theory proves insufficient. This theoretical framework and numerical evaluation motivate the inclusion of unsteady flow models in design and simulation tools in order to increase the robustness and operational lifespans of wind turbine blades in real flow conditions.

==> unused_text.tex <==
%We then investigate the extent to which the theoretical predictions can capture the range of dynamics allowable within the assumptions of a blade-element approach.

% provide predictive capabilities for applications in deploying highly flexible structures that may encounter gusts. 

% When considering a pitching and plunging airfoil in a periodic transverse gust, these effects are often treated separately in theory while they appear together in practice.

%This theoretical framework and numerical validation provide predictive capabilities for applications such as gust-load alleviation for increased robustness against fatigue and the optimization of flapping flight in gusty environments for enhanced maneuverability and control authority.

% \textcolor{red}{NOTES}

% \begin{enumerate}
    % \item NEW TITLE NEEDED
    % \item Reframe along the lines of 2D unsteady extension to BEM solvers (Qblade?)
    % \item QBlade uses empirical corrections (dynamic inflow model, see Hendriksen et al. 2012)
    % \item Our thing could be used as an additional correction
    % \item Cite QBlade and FVW papers (e.g. de Vaal) to demonstrate that dynamic inflow models are the standard
    % \item Our modeling approach bridges the gap between 2D BEM approaches without fundamental unsteady physics and unsteady aerodynamics theory / modeling - can bring in effects like thickness, camber, 3D effects, etc.
    % \item if we care about sectional 2D physics in BEM, then we should reexamine the fundamentals and then add in corrections (word choice not optimal) to make it fully applied
    % \item Defend use of Sears + Theodorsen by wind-turbine aerodynamics: yawed turbines experience Sears conditions (even in steady flow), and large turbines have aeroelastic blade oscillations (Theodorsen), so combination is important
% \end{enumerate}

% Things to prune 

% \begin{enumerate}
    % \item Section 2: Remove most of derivation of Sears and Theodorsen and skip right to current equation (9)
    % \item Note: don't need to reiterate much that more advanced corrections exist - just in one sentence or so
    % \item Waveform plots in section 4.1: condense into 3-up, remove 2 legends
    % \item Waveform plots (theory vs simulation) - make smaller and 3 in a row, remove legend from all but one
    % \item Figures 8-12 can be made squatter, and remove text from axes (only variables)
    % \item Conclusions: 2nd paragraph focused only on 2D BEM codes, rephrase last paragraph for more wind-turbine vibes, and add in text about how this could be used for LLT since it depends on the same 2D sectional information as classical BEM
    % \item Be judicious about what to reference
% \end{enumerate}

% Additionally, the numerical framework allows these dynamics to be studied at very high reduced frequencies, considering reduced frequencies based on the airfoil-oscillation frequency of $k_p = 0.785$ and impinging gust-based reduced frequencies of up to $k_g = 3.93$. \textcolor{red}{Should we add wind-turbine context here or down in Section 3 where we state the actual ranges and talk about Strouhal number as well? Maybe this sentence isn't even necessary...}


% The unsteady aerodynamics of oscillating bodies in gusty environments are highly relevant to several applications in aeronautical, biological, and environmental contexts. While natural flapping fliers, such as birds and insects, can easily manipulate the interaction of oscillating wings and atmospheric gusts to enhance their maneuverability, human-engineered systems often fare worse when subjected to gusts and induced oscillations. Wind-turbine blades, aircraft wings, helicopter rotor blades, and other structures exposed to the atmosphere are becoming larger and lighter due to improvements in materials and fabrication technologies. This size leads to increased flexibility and aeroelastic effects, which in turn make these moving components particularly sensitive to gust disturbances, as unsteady loads from an impinging gust can initiate forced structural oscillations that can result in increased fatigue loading, decreased operational lifespans, and in extreme cases, catastrophic failure. This is an especially critical problem for the design and control of uncrewed aerial vehicles (UAVs) and micro air vehicles (MAVs), which often operate in conditions where the velocities associated with atmospheric fluctuations are similar in magnitude to flight speeds and are therefore strongly affected by gust disturbances \citep{jones_physics_2022}.


% The Sears function has been extensively validated in experiments \citep[e.g.][]{li_direct_2018, wei_insights_2019}, and has generally been shown to represent the lift response of a sufficiently thin airfoil well at relatively low reduced frequencies ($k_g \lesssim 1$) \citep{lysak_measurement_2016, li_aerodynamic_2022}. These studies have shown that the effects of airfoil thickness become non-negligible at higher reduced frequencies, leading to an overprediction of the lift-response magnitude. Similarly, the Theodorsen problem has been studied over a wide range of conditions, including at large amplitudes where significant flow separation occurs and the airfoil undergoes dynamic stall \citep{visbal_investigation_1989, ol_shallow_2010, baik_experimental_2012, rival_characteristic_2014}. However, even within the attached-flow regime, \citet{taha_viscous_2019} suggest that viscous effects lead the theory to overpredict both magnitude and phase of the unsteady lift response of a pitching airfoil at reduced frequencies approaching unity. \citet{catlett_unsteady_2020} have shown a similar overprediction at reduced frequencies exceeding unity in simulations involving small-amplitude pitching motions and airfoils of differing thicknesses. Still, even in the dynamic-stall regime, the Theodorsen function is capable of qualitatively capturing the lift response of pitching and plunging foils \citep{baik_unsteady_2012}. Hence, both the Sears and Theodorsen models can yield helpful insights into the unsteady aerodynamics of structures in gusts and oscillatory motions, even when some of their foundational assumptions are violated.

%To demonstrate the validity of this approach, as well as to serve as a resource for further generalizations of these analytical models for arbitrary disturbances, we present a brief overview of the derivation to directly demonstrate the linearity of the problem.

%\citet{von_karman_airfoil_1938} provide a general method for determining the unsteady lift on an airfoil if the vertical velocity at every point on the airfoil surface is known. The lift is given by the expression

%\begin{equation}
%L=-\rho \frac{d}{dt}\int_{-1}^{1} \gamma_0(x) x dx + \rho U_\infty \Gamma_0 + \rho U_\infty \int_{1}^\infty \gamma(\xi) \frac{d\xi}{\sqrt{\xi^2-1}},
%\label{eqn:L_gamma}
%\end{equation}

%\noindent where $x$ is the nondimensional streamwise coordinate on the airfoil \textcolor{black}{(unitized in half-chords)} and $\xi$ is the streamwise coordinate in the wake. The parameters $\gamma_0$, $\Gamma_0$, and $\gamma$ represent circulation contributions to the total lift from motions of the airfoil, the quasi-steady airfoil circulation, and the distribution of vorticity in the wake, respectively. The three components thus correspond to an added-mass force, a quasi-steady lift force, and the induced circulatory force from the wake. Since each of the lift contributions depends linearly on the circulation, in keeping with the potential-flow origins of the theoretical framework, Equation \ref{eqn:L_gamma} justifies the superposition of multiple disturbances by adding the relevant circulations.

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figs/AoA_CL_PPG3}
    \caption{Time-varying quantities from a sample case with $f_g/f_p=1$, $\hat{\alpha}_g=\hat{\theta}=3^\circ$, and $\hat{h}/c=0.03$. Top: Net angle of attack at the airfoil quarter-chord point (blue) and contributions from pitch, plunge, and gust oscillations (orange, gold, and green). Bottom: Theoretical prediction of the time-varying lift coefficient (blue) compared with the phase-averaged simulation data (red), with Theodorsen and Sears contributions (grey).}
    \label{fig:AoA_PPG3}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figs/AoA_CL_FR4A3}
    \caption{Time-varying quantities from a sample case with $f_g/f_p=4$, $\hat{\alpha}_g=\hat{\theta}=3^\circ$, and $\hat{h}/c=0.03$. Top: Net angle of attack at the airfoil quarter-chord point (blue) and contributions from pitch, plunge, and gust oscillations (orange, gold, and green). Bottom: Theoretical prediction of the time-varying lift coefficient (blue) compared with the phase-averaged simulation data (red), with Theodorsen and Sears contributions (grey).}
    \label{fig:AoA_FR4A3}
\end{figure}

%This of course will not be the case for forcing conditions with other phase relationships between the gust, pitch, and plunge disturbances.

% In Figure \ref{fig:AoA_FR025A3}, we plot the computed angles of attack ($\alpha$) for an FR case where $f_g/f_p = 0.25$, . For this case, we see that the simulation results for net lift compare quite favorably with the theoretical prediction. The complexity of the angle-of-attack variations and the differences between the individual predictions of the Sears and Theodorsen theories emphasize that, even when the forcing frequencies are relatively distinct, both gust and airfoil-oscillation contributions must be accounted for to correctly model the lift response in this problem.

% Again, the simulation results appear to be well-described by the proposed model, which \textcolor{black}{so far} supports the conjecture that the model can effectively capture the lift response across a range of forcing frequencies, amplitudes, and phase relations.

% In Figure \ref{fig:AoA_FR4A3}, we now consider an FR case with $f_g/f_p = 4$, where the amplitudes of the forcings remain identical to the previous two cases. As 

% This study demonstrates the capacity of simple models of unsteady aerodynamics to capture superpositions of dynamics in the linear regime. It is therefore highly relevant for the modeling and control of light aircraft, UAVs, MAVs, and small wind turbines that operate in highly unsteady flow environments. The transfer-function formulation of the model is particularly well-suited for the design of controllers that can manipulate airfoil-oscillation kinematics to achieve either gust-load alleviation or lift enhancement in propulsion contexts. Even outside of the linear regime, the model form could be adapted with empirical coefficients for control applications, as has been done by \citet{brunton_empirical_2013} for the pure Theodorsen problem. These efforts may yield insights into the ways in which birds, insects, and other flying animals leverage flow unsteadiness for enhanced maneuverability and robustness in flight.

%The three-dimensionality of the complete problem and its turbulent implications could also be studied in a similar framework as the setups in \citet{negi_unsteady_2018} and \citet{yang_three-dimensional_2019}. The problem of controlling incipient separation and dynamic stall, for example, could benefit from such work. The effects of finite aspect ratio on the model predictions, as well as their effects on the dynamic-stall process at higher perturbation amplitudes, could also be studied in detail. Three-dimensional flow interactions at the airfoil tips may be of significant interest for both the lift of the oscillating wing as it encounters a gust and the evolution of its wake, which would affect the performance of other aerodynamic profiles downstream.

%\textcolor{black}{First, in Figure \ref{fig:polar}, we plot the variation in the steady-state lift coefficient with inflow angle of attack, along with the theoretical lift profile from 2D thin-airfoil theory at low angles of attack. At low angles of attack,  ($\alpha \lesssim 3^\circ$), the simulation data match the analytic results quite well, whereas at higher angles of attack, some differences between the two frameworks are observed. We also found that the data agreed well with values provided by a standard aerodynamic tool, XFOIL, in the zero-Mach limit with matching chord-based Reynolds number \citep{drela_xfoil:_1989}.} The influence of unsteady phenomena such as flow separation and vortex shedding is visible in the higher variance in the simulation results at angles of attack exceeding $\alpha \approx 10^\circ$. Still, it is important to reiterate here that since we are most interested in comparison with inviscid theory (in which turbulent eddies are not present), we do not seek to fully resolve the smallest of the near-wall structures. Furthermore, as we restrict ourselves to a two-dimensional domain, the turbulence modeled in these simulations will not have energetics identical to that produced in the equivalent three-dimensional setup \cite[cf.][]{kraichnan_inertial_1967}. So long as the instantaneous angle of attack in our simulations stays well below $\alpha=10^\circ$, we should avoid regimes where separation effects are non-negligible. 

% \subsection{Baseline Validation Study}

%To build confidence in our approach and the NaluCFD solver, two validation studies were carried out.

%\begin{figure}[t]
%    \centering
    %\includegraphics[width=0.6\textwidth]{figs/CL_steady_polar}
    %\caption{Steady lift coefficient ($C_l$) vs. angle of attack ($\alpha$) for the NACA-0012 airfoil. Simulation data at $Re_c=2.22\times10^5$ are plotted as red squares, and are compared with the ideal lift profile from 2D thin-airfoil theory (blue dashed line). \textcolor{red}{REMOVE along with associated discussion.}}
    %\label{fig:polar}
%\end{figure}


%%% TEMPLATE %%%

%% Since the Copernicus LaTeX package includes the BibTeX style file copernicus.bst,
%% authors experienced with BibTeX only have to include the following two lines:
%%
%% \bibliographystyle{copernicus}
%% \bibliography{example.bib}
%%
%% URLs and DOIs can be entered in your BibTeX file as:
%%
%% URL = {http://www.xyz.org/~jones/idx_g.htm}
%% DOI = {10.5194/xyz}


%% LITERATURE CITATIONS
%%
%% command                        & example result
%% \citet{jones90}|               & Jones et al. (1990)
%% \citep{jones90}|               & (Jones et al., 1990)
%% \citep{jones90,jones93}|       & (Jones et al., 1990, 1993)
%% \citep[p.~32]{jones90}|        & (Jones et al., 1990, p.~32)
%% \citep[e.g.,][]{jones90}|      & (e.g., Jones et al., 1990)
%% \citep[e.g.,][p.~32]{jones90}| & (e.g., Jones et al., 1990, p.~32)
%% \citeauthor{jones90}|          & Jones et al.
%% \citeyear{jones90}|            & 1990



%% FIGURES

%% When figures and tables are placed at the end of the MS (article in one-column style), please add \clearpage
%% between bibliography and first table and/or figure as well as between each table and/or figure.

% The figure files should be labelled correctly with Arabic numerals (e.g. fig01.jpg, fig02.png).


%% ONE-COLUMN FIGURES

%%f
%\begin{figure}[t]
%\includegraphics[width=8.3cm]{FILE NAME}
%\caption{TEXT}
%\end{figure}
%
%%% TWO-COLUMN FIGURES
%
%%f
%\begin{figure*}[t]
%\includegraphics[width=12cm]{FILE NAME}
%\caption{TEXT}
%\end{figure*}
%
%
%%% TABLES
%%%
%%% The different columns must be seperated with a & command and should
%%% end with \\ to identify the column brake.
%
%%% ONE-COLUMN TABLE
%
%%t
%\begin{table}[t]
%\caption{TEXT}
%\begin{tabular}{column = lcr}
%\tophline
%
%\middlehline
%
%\bottomhline
%\end{tabular}
%\belowtable{} % Table Footnotes
%\end{table}
%
%%% TWO-COLUMN TABLE
%
%%t
%\begin{table*}[t]
%\caption{TEXT}
%\begin{tabular}{column = lcr}
%\tophline
%
%\middlehline
%
%\bottomhline
%\end{tabular}
%\belowtable{} % Table Footnotes
%\end{table*}
%
%%% LANDSCAPE TABLE
%
%%t
%\begin{sidewaystable*}[t]
%\caption{TEXT}
%\begin{tabular}{column = lcr}
%\tophline
%
%\middlehline
%
%\bottomhline
%\end{tabular}
%\belowtable{} % Table Footnotes
%\end{sidewaystable*}
%
%
%%% MATHEMATICAL EXPRESSIONS
%
%%% All papers typeset by Copernicus Publications follow the math typesetting regulations
%%% given by the IUPAC Green Book (IUPAC: Quantities, Units and Symbols in Physical Chemistry,
%%% 2nd Edn., Blackwell Science, available at: http://old.iupac.org/publications/books/gbook/green_book_2ed.pdf, 1993).
%%%
%%% Physical quantities/variables are typeset in italic font (t for time, T for Temperature)
%%% Indices which are not defined are typeset in italic font (x, y, z, a, b, c)
%%% Items/objects which are defined are typeset in roman font (Car A, Car B)
%%% Descriptions/specifications which are defined by itself are typeset in roman font (abs, rel, ref, tot, net, ice)
%%% Abbreviations from 2 letters are typeset in roman font (RH, LAI)
%%% Vectors are identified in bold italic font using \vec{x}
%%% Matrices are identified in bold roman font
%%% Multiplication signs are typeset using the LaTeX commands \times (for vector products, grids, and exponential notations) or \cdot
%%% The character * should not be applied as mutliplication sign
%
%
%%% EQUATIONS
%
%%% Single-row equation
%
%\begin{equation}
%
%\end{equation}
%
%%% Multiline equation
%
%\begin{align}
%& 3 + 5 = 8\\
%& 3 + 5 = 8\\
%& 3 + 5 = 8
%\end{align}
%
%
%%% MATRICES
%
%\begin{matrix}
%x & y & z\\
%x & y & z\\
%x & y & z\\
%\end{matrix}
%
%
%%% ALGORITHM
%
%\begin{algorithm}
%\caption{...}
%\label{a1}
%\begin{algorithmic}
%...
%\end{algorithmic}
%\end{algorithm}
%
%
%%% CHEMICAL FORMULAS AND REACTIONS
%
%%% For formulas embedded in the text, please use \chem{}
%
%%% The reaction environment creates labels including the letter R, i.e. (R1), (R2), etc.
%
%\begin{reaction}
%%% \rightarrow should be used for normal (one-way) chemical reactions
%%% \rightleftharpoons should be used for equilibria
%%% \leftrightarrow should be used for resonance structures
%\end{reaction}
%
%
%%% PHYSICAL UNITS
%%%
%%% Please use \unit{} and apply the exponential notation

%% The following commands are for the statements about the availability of data sets and/or software code corresponding to the manuscript.
%% It is strongly recommended to make use of these sections in case data sets and/or software code have been part of your research the article is based on.
